G-Refer: Graph Retrieval-Augmented Large Language Model for Explainable Recommendation

Explainable recommendation has demonstrated significant advantages in informing users about the logic behind recommendations, thereby increasing system transparency, effectiveness, and trustworthiness. To provide personalized and interpretable explanations, existing works often combine the generation capabilities of large language models (LLMs) with collaborative filtering (CF) information. CF information extracted from the user-item interaction graph captures the user behaviors and preferences, which is crucial for providing informative explanations. However, due to the complexity of graph structure, effectively extracting the CF information from graphs still remains a challenge. Moreover, existing methods often struggle with the integration of extracted CF information with LLMs due to its implicit representation and the modality gap between graph structures and natural language explanations. To address these challenges, we propose G-Refer, a framework using graph retrieval-augmented large language models (LLMs) for explainable recommendation. Specifically, we first employ a hybrid graph retrieval mechanism to retrieve explicit CF signals from both structural and semantic perspectives. The retrieved CF information is explicitly formulated as human-understandable text by the proposed graph translation and accounts for the explanations generated by LLMs. To bridge the modality gap, we introduce knowledge pruning and retrieval-augmented fine-tuning to enhance the ability of LLMs to process and utilize the retrieved CF information to generate explanations. Extensive experiments show that G-Refer achieves superior performance compared with existing methods in both explainability and stability. Codes and data are available at https://github.com/Yuhan1i/G-Refer.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/challenges.tex <==
\section{Existing Limitations}

% \noindent \textbf{Knowledge-unaware}

\noindent \textbf{Implicit Collorative Signal.}

% 为什么和RAG结合进来？

\noindent \textbf{Lacking}

% 为什么要双路retrieval？

% Insufficient Global/Long-Range Information

% why graph rag

\noindent \textbf{Irrelevant Training Samples.}

==> tables/hyper_numbers.tex <==
\begin{table}[t]
\centering
\caption{Hyperparameter study of knowledge pruning ratio $k$.}
\label{tab:hyper_k}
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{l|ccc}
\toprule
\multirow{2}{*}{\textbf{Ratio}} & \multicolumn{3}{c}{\textbf{Explainability $\uparrow$}} \\
\cmidrule(lr){2-4} 
 & Precision & Recall & F1-score  \\
\midrule

\multicolumn{4}{c}{\textbf{Amazon-books}} \\
\midrule
$k$=1 & 40.71 & 44.49  &  42.52  \\
$k$=2 & 40.73 & 44.94  &  42.89  \\
$k$=3 & 40.43 &  44.44 &  42.34 \\
$k$=4 & 40.13 &  44.29 &  42.11  \\
$k$=5 & 40.22 & 44.54  & 42.27  \\

\midrule

\multicolumn{4}{c}{\textbf{Yelp}} \\
\midrule
$k$=1 & 36.18 &  43.77 & 39.61  \\
$k$=2 & 36.29 & 43.73  & 40.03 \\
$k$=3 & 36.11 & 43.67  & 39.53 \\
$k$=4 & 36.10 & 43.70  & 39.54  \\
$k$=5 & 35.89 &  43.79 & 39.45 \\


\midrule

\multicolumn{4}{c}{\textbf{Google-reviews}} \\
\midrule
$k$=1 & 41.82 & 49.24  & 45.23  \\
$k$=2 & 42.45 & 49.35  & 45.92  \\
$k$=3 & 41.87 & 49.38  & 45.32   \\
$k$=4 & 41.34 &  49.38 &  45.00 \\
$k$=5 & 40.21 & 49.23  & 44.26   \\

\bottomrule
\end{tabular}
}
\end{table}

==> tables/hyper_ratio.tex <==
\begin{table}[t]
\centering
\caption{Performance of different knowledge pruning ratio $t$.}
\label{tab:hyper_t}
\resizebox{0.85\columnwidth}{!}{
\begin{tabular}{l|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Pruning Ratio}} & \multicolumn{2}{c|}{\textbf{Explainability $\uparrow$}} & \multicolumn{2}{c}{\textbf{Stability $\downarrow$}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & \textbf{BERT${^\text{F1}}$} & \textbf{BLEURT}  & \textbf{BERT${_\text{std}}$} & \textbf{BLEURT${_\text{std}}$} \\
\midrule

\multicolumn{5}{c}{\textbf{Amazon-books}} \\
\midrule
$t$=90\% & 0.4211 & -0.1388 & \textbf{0.0817} & \underline{0.1905} \\
$t$=80\% & 0.4253 & -0.1339 & 0.0821 & 0.1913 \\
$t$=70\% & \textbf{0.4289} & \textbf{-0.1203} & 0.0825 & 0.1912 \\
$t$=60\% & \underline{0.4279} & \underline{-0.1263} & 0.0830 & 0.1910 \\
$t$=50\% & 0.4255 & -0.1326 & \underline{0.0819} & \textbf{0.1893} \\

\midrule

\multicolumn{5}{c}{\textbf{Yelp}} \\
\midrule
$t$=90\% & \underline{0.3974} & \underline{-0.1455} & 0.0872 & 0.2240 \\
$t$=80\% & 0.3961 & -0.1458 & 0.0866 & 0.2207 \\
$t$=70\% & \textbf{0.4003} & \textbf{-0.1335} & 0.0885 & 0.2182 \\
$t$=60\% & 0.3927 & -0.1461 & \underline{\textbf{0.0856}} & \underline{0.2178} \\
$t$=50\% & 0.3967 & -0.1461 & \underline{\textbf{0.0856}} & \textbf{0.2164} \\

\midrule

\multicolumn{5}{c}{\textbf{Google-reviews}} \\
\midrule
$t$=90\% & 0.4462 & -0.1798 & 0.0919 & 0.2437 \\
$t$=80\% & 0.4518 & -0.1645 & 0.0927 & 0.2508 \\
$t$=70\% & \underline{0.4592} & -0.1517 & \underline{0.0916} & 0.2511 \\
$t$=60\% & 0.4583 & \underline{-0.1465} & 0.0918 & \textbf{0.2477} \\
$t$=50\% & \textbf{0.4606} & \textbf{-0.1459} & \textbf{0.0907} & \underline{0.2498} \\

\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table}
